Evidence of electronic states driving current-induced insulator-to-metal transition

On demand current-driven insulator-to-metal transition (IMT) is pivotal for the next generation of energy-efficient and scalable microelectronics. IMT is a key phenomenon observed in various quantum materials, and it is enabled by the complex interplay of spin, lattice, charge, and orbital degrees of freedom (DOF). Despite significant prior work, the underlying mechanism of the current-driven IMT remains elusive, primarily due to the difficulty in simultaneously obtaining bulk fingerprints of all the electronic DOF. Here, we employ in-operando resonant inelastic x-ray scattering (RIXS) on Ca$_2$RuO$_4$, a prototypical strongly correlated material, to track the evolution of the electronic DOF encoded in the RIXS spectra during the current-driven IMT. Upon entering the conductive state, we observe an energy-selective suppression of the RIXS intensity, proportional to the current. Using complementary RIXS cross-section calculations, we demonstrate that the non-equilibrium conductive state emerges from the formation of correlated electronic states with a persistent Mott gap.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }

}
